Memory Consolidation Enables Long-Context Video Understanding

Most transformer-based video encoders are limited to short temporal contexts due to their quadratic complexity. While various attempts have been made to extend this context, this has often come at the cost of both conceptual and computational complexity. We propose to instead re-purpose existing pre-trained video transformers by simply fine-tuning them to attend to memories derived non-parametrically from past activations. By leveraging redundancy reduction, our memory-consolidated vision transformer (MC-ViT) effortlessly extends its context far into the past and exhibits excellent scaling behavior when learning from longer videos. In doing so, MC-ViT sets a new state-of-the-art in long-context video understanding on EgoSchema, Perception Test, and Diving48, outperforming methods that benefit from orders of magnitude more parameters.

==> algorithms/memory_consolidation.tex <==
\begin{algorithm}[t]
\caption{Memory consolidation methods.}
\label{alg:mc_algorithm}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{ouralg!20},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
}
\begin{lstlisting}[language=python]
def memory_consolidation(
              memory, activations, k, method):
    random_indices = np.random.uniform(
        low=0, high=activations.shape[1], size=k)
    random_k_activations = activations[random_indices]
    if method == 'cross_attention':
      q = random_k_activations
      kv = np.concatenate([activations, memory],axis=1)
      weights = L2_similarity(q, kv)
      weights = softmax(weights, axis=-1)
      memory_t = np.einsum('bmn,bnd->bmd', weights, kv)
    elif method == 'kmeans':
      centroids = random_k_activations
      memory_t = k_means(centroids, embeddings)
    elif method == 'random':
      memory_t = random_k_activations
  return np.concatenate([memory, memory_t], axis=1)
\end{lstlisting}
\end{algorithm}

%   # Inputs:
%   #   memory: consolidated past memory, of shape
%   #   [batch_size, mem_len, D].
%   #   activations: embeddings of current observation,
%   #   of shape [batch_size, emb_len, D].
%   #   k: size of consolidated memory for current chunk.
%   #   method: memory consolidation method to use, choose
%   #   between 'cross_attention', 'kmeans', 'random'.
%   #
%   # Returns:
%   #   Consolidated memory for current time step.

==> tables/table_num_frames.tex <==
\begin{table}[t]
\caption{\textbf{Benchmarks.} Default settings for training and evaluation per dataset. 
}
\label{tab:benchmarks}
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
Dataset & Avg Length & \multirow{2}{*}{\shortstack{Frame\\sampling}} & \multicolumn{2}{c}{Frames} \\
\cmidrule(lr){4-5}
& &  & Train & Eval \\
\midrule
Diving48 &  \\ 
EgoSchema & 180 sec & Uniformly & 64 & 128 \\ 
NextQA & 44 sec & Uniformly & 64 & 128 \\ 
Perception Test & 30 sec & 4 FPS & 64 & 256 \\ 
\end{tabular}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}

